Improving Non-autoregressive Translation Quality with Pretrained Language Model, Embedding Distillation and Upsampling Strategy for CTC

Non-autoregressive approaches aim to improve the inference speed of translation models, particularly those that generate output in a one-pass forward manner. However, these approaches often suffer from a significant drop in translation quality compared to autoregressive models. This paper introduces a series of innovative techniques to enhance the translation quality of Non-Autoregressive Translation (NAT) models while maintaining a substantial acceleration in inference speed. We propose fine-tuning Pretrained Multilingual Language Models (PMLMs) with the CTC loss to train NAT models effectively. Furthermore, we adopt the MASK insertion scheme for up-sampling instead of token duplication, and we present an embedding distillation method to further enhance performance. In our experiments, our model outperforms the baseline autoregressive model (Transformer \textit{base}) on multiple datasets, including WMT'14 DE$\leftrightarrow$EN, WMT'16 RO$\leftrightarrow$EN, and IWSLT'14 DE$\leftrightarrow$EN. Notably, our model achieves better performance than the baseline autoregressive model on the IWSLT'14 En$\leftrightarrow$De and WMT'16 En$\leftrightarrow$Ro datasets, even without using distillation data during training. It is worth highlighting that on the IWSLT'14 DE$\rightarrow$EN dataset, our model achieves an impressive BLEU score of 39.59, setting a new state-of-the-art performance. Additionally, our model exhibits a remarkable speed improvement of 16.35 times compared to the autoregressive model.

==> chaps/ethical.tex <==
\section{Ethical Concerns} \label{ethical}
Although our NAT models, datasets and AT teachers are from publicly-available resources, there may be some intrinsic bias in all of them. Some may thus be harmful to potential users. To alleviate this problem, we can seek refinement frameworks or security risk detectors to modify or remove risk sentences or words.

==> chaps/intro.tex <==

\section{Introduction} \label{intro}
Autoregressive machine Translation (AT) \cite{mikolov2010recurrent,bahdanau2014neural,vaswani2017attention} models have long been the state-of-the-arts on various translation tasks, but one of the major drawbacks is not efficiently parallelizable on GPU or TPU during inference. To solve this problem, the prior work \cite{Gu0XLS18} proposed the Non-Autogressive machine Translation (NAT) models, which can generate all target tokens in parallel. While the speedup is significant, NAT suffers from degraded generation quality compared to AT models.

% One of the limitations of NAT models is the tradeoff between generation iterations and translation quality \cite{gu-kong-2021-fully}. Since the advance of CTC-based NAT models \cite{saharia-etal-2020-non,gu-kong-2021-fully,shao-etal-2022-one,shao2022nmla}, NAT models can now generate translations of high quality in a single iteration without the need for length prediction. On the other hand, it has been shown that Pretrained Language Models (PLM) are beneficial for for CMLM-based \cite{ghazvininejad-etal-2019-mask} iterative NAT models, either by integrating into the model architecture \cite{10.5555/3495724.3496634} or by pretrain a PLM anew \cite{li-etal-2022-universal}. Thus incorporating PLMs into CTC-based NAT models may also lift their performance to a next level.

To improve the quality of NAT, the previous works \cite{10.5555/3495724.3496634,li-etal-2022-universal} use Pretrained Language Models (PLM) to initialize the NAT with CMLMs \cite{ghazvininejad-etal-2019-mask} architecture. However, they need more iterations to achieve better performance and exist a problem of accuracy of predicting length. Additionally, one popular solution to solve the tradeoff between generation iterations and translation quality \cite{gu-kong-2021-fully} is the CTC-based NAT models \cite{libovicky-helcl-2018-end, saharia-etal-2020-non,gu-kong-2021-fully,shao-etal-2022-one,shao2022nmla} that generate translations of high quality in a single iteration without length prediction.

In this paper, we propose a new model named CTCPMLM to combine encoder-based PMLMs with CTC loss in training NAT models to see whether PMLMs can further boost a CTC NAT model’s performance. To leverage the natural language capabilities of PMLM, we distill target sentences from PMLM to guide the NAT student model to learn more realistic embedding. Furthermore, the source embedding needs to upsample to feed into the model for CTC loss, most of the upsampling ratio can only be an integer value, and the fixed upsampling ratio is dominated by the longest sentence.  To alleviate this problem, we propose a dynamic ratio to adjust the ratio for each sentence dynamically. \\
In summary, our contributions are: \\
\begin{itemize}
    \item Unlike previous works \cite{rothe-etal-2020-leveraging, 10.5555/3495724.3496634, Zhu2020Incorporating,su-etal-2021-non} that incorporates PMLMs with additional modules, we directly finetune PMLMs with CTC without introducing additional parameters, proving it is an efficient and effective method in experiments.
\end{itemize}

\begin{itemize}
    \item We propose a new upsampling scheme of inserting "MASK" tokens and an adaptive upsampling rate that further increases the performance of our NAT models. We also conduct a thorough search on different upsampling schemes to make the model achieve better accuracy.
\end{itemize}

\begin{itemize}
    \item We propose to distill the knowledge from a frozen PMLM in the contextualized embedding level as a regularization method for our NAT model to retain the target language information learned from pretraining.
\end{itemize}

\begin{itemize}
    \item Our models perform on par with baseline AT models on IWSLT'14 En$\leftrightarrow$De and WMT'16 En$\leftrightarrow$Ro even on the raw data (undistilled training set).
\end{itemize}



==> chaps/intro_long.tex <==
\section{Introduction} \label{intro}
\IEEEPARstart{A}{utoregressive} (AT) machine translation\cite{mikolov2010recurrent,bahdanau2014neural,vaswani2017attention} models have long been the state-of-the-arts on various translation tasks, but one of the major drawbacks is not efficiently parallelizable on GPU or TPU during inference. To solve this problem, the prior work \cite{Gu0XLS18} proposed the non-autoregressive neural machine translation (NAT) models, which can generate all target tokens in parallel. While the speedup is significant, NAT suffers from degraded generation quality compared to AT models.

One of the main challenges is determining the appropriate target sequence length in advance. In the case, \cite{Gu0XLS18} employs Noisy Parallel Decoding (NPD), which generates multiple predictions of different lengths with fertility, and then a pretrained AT model is used to rescore them. \cite{stern19a,GuWZ19}  applied insertion method, which is partially autoregressive and uses the insertion operations for more flexible and dynamic length changes. \cite{shu2020latent} refines the latent variables instead of the tokens, allowing for dynamically adaptive prediction length. One popular solution is the CTC-based NAT models \cite{libovicky-helcl-2018-end, saharia-etal-2020-non,gu-kong-2021-fully,shao-etal-2022-one,shao2022nmla}, which introduces connectionist temporal classification (CTC) \cite{GravesFGS06} to solve the target length problem. 
% In this work, we employ the CTC loss and propose the CTC upsampling strategy to further enhance performance.

Another main challenge is the multi-modality problem. NAT removes the conditional dependence between target tokens, and predicting the independent issue leads to multi-modal outputs and induces the repetition of tokens \cite{Gu0XLS18,zhou2021understanding}. A standard approach to overcome the multi-modality problem is to use sequence-level knowledge distillation \cite{kim-rush-2016-sequence}, by replacing the target side of the training set with the output from an AT model. Various advanced model architectures \cite{lee-etal-2018-deterministic,ghazvininejad-etal-2019-mask} use iteration-based methods that can see the previous or partially predicted tokens to add dependence to solve the multi-modality problem.
% This work explores an alternative paradigm: we use not only strong AT teacher in sequence-level knowledge distillation but also leverage contextualized PMLM in target to learn the information from pertaining.

There have been some pretrained encoder-decoder-based multilingual language models \cite{lample2019cross,zanon-boito-etal-2020-mass,liu-etal-2020-multilingual-denoising,xue-etal-2021-mt5,li-etal-2022-universal} that achieve superior translation performance. Most of them are dedicated to AT, while \cite{li-etal-2022-universal} intends to pretrain models that can be applied to both AT and NAT. Some \cite{rothe-etal-2020-leveraging, lample2019cross, Zhu2020Incorporating, 10.5555/3495724.3496634} otherwise incorporate encoder-based pretrained multilingual language models (PMLMs) into encoder-decoder-based transformer AT models for better translation performance. \cite{li-etal-2022-universal, Zhu2020Incorporating, 10.5555/3495724.3496634,su-etal-2021-non} utilizes PMLMs to initialize NAT models. Among them, \cite{li-etal-2022-universal, Zhu2020Incorporating, 10.5555/3495724.3496634} are iterative models with strong performance while \cite{su-etal-2021-non} is one-pass with weaker performance.
% This work instead directly finetunes PMLMs with CTC as one-pass models for faster inference, yet with comparable or better performance with respect to PMLM-initialized iterative NAT models.

Previous research \cite{hinton2015distilling, tang2019distilling, sanh2020distilbert} has shown the effectiveness of knowledge distillation in transferring knowledge from complex models to smaller student models. These studies have demonstrated that a student model can benefit from a teacher model's knowledge by learning from its softened probabilities. Motivated by these findings, we leverage knowledge distillation to enhance the translation performance of our NAT model. Our specific focus is on utilizing the rich semantic and contextual information encoded in the embedding space of a PMLM to improve the quality of translations

% Based on the aforementioned findings, our objective is to integrate these techniques and propose a novel method to enhance the performance of NAT. This paper introduces CTCPMLM, a one-pass NAT approach that combines the utilization of encoder-based PMLMs for model initialization and the integration of CTC loss. We introduce a CTC upsampling strategy to enhance performance. Furthermore, our approach not only incorporates a strong AT teacher in sequence-level knowledge distillation but also leverages contextualized PMLMs in the target side to acquire embedding-level information from PMLM. \\

Based on the aforementioned findings, our goal is to integrate these techniques and propose a novel method to enhance the performance of NAT. In this paper, we introduce CTCPMLM, a one-pass NAT approach that combines the utilization of encoder-based PMLMs for model initialization and the integration of the CTC loss with sequence-level knowledge distillation using a strong AT teacher. Additionally, we propose a CTC upsampling strategy to address the fixed rate problem and improve performance by inserting "MASK" tokens. Furthermore, we leverage knowledge distillation for embedding distillation, specifically distilling the embeddings from the target language layer of the PMLM. Moreover, we employ bipartite matching to solve the embedding alignment problem between the source and target languages.



In summary, our contributions are: 
\begin{itemize}
    \item Unlike previous works \cite{rothe-etal-2020-leveraging, 10.5555/3495724.3496634, Zhu2020Incorporating,su-etal-2021-non} that incorporates PMLMs with additional modules, we directly finetune PMLMs with CTC without introducing additional parameters, verifying it is an efficient and effective method in experiments.

    \item We propose a new upsampling scheme of inserting "MASK" tokens and an adaptive upsampling rate that further increases the performance of our NAT models. We also conduct a thorough search on different upsampling schemes to make the model achieve better accuracy.

    \item We propose to distill the knowledge from a frozen PMLM in the contextualized embedding level as a regularization method for our NAT model to retain the target language information learned from pretraining.
    
    \item Our model surpasses the baseline of the auto-regressive model (Transformer \textit{base}) on WMT'14 DE$\leftrightarrow$EN, WMT'16 RO$\leftrightarrow$EN, and IWSLT'14 DE$\leftrightarrow$EN datasets and speed improvement of 16.35 times compared to the auto-regressive model.

    \item Our model achieves a BLEU score of 39.59 on IWSLT'14 DE$\rightarrow$EN, which is a new state-of-the-art performance. It is worth noting that our performance surpasses that of baseline AT models even on IWSLT'14 En$\leftrightarrow$De and WMT'16 En$\leftrightarrow$Ro datasets, even when trained on the raw data (undistilled training set).
\end{itemize}


==> chaps/limitations.tex <==

\section{Limitations} \label{limiations}
An important limitation of CTCPMLM is that not every language pair have a bi-lingual PLM pretrained on it. Since according to TABLE \ref{tab:diff_pmlm} the most outstanding PMLM is the bi-lingual LM BiBERT, for other language pairs without a PLM exclusively pretrained on it, the performance with other readily available PMLMs may not be optimal. Also, it may be unaffordable to pretrain a bi-lingual PLM for every single language pair. Another limitation is the vocabulary of each PMLM. If a PMLM does not support uppercase words, it will limit CTCPMLM to only output lowercase translations. Again, this will induce the need of a new PMLM with cased vocabulary. Lastly, our models are trained on only three standard machine translation datasets for only a single run, which suggests that we need to train our models on more datasets for more runs for results of statistical significance. 
%, so it is necessary to add a model or function to do proper uppercase processing.

==> chaps/related_work.tex <==
\section{Related Work} \label{relatedwork}
\subsection{Length Prediction}
One of the main challenges lies in ensuring the accuracy of the target sequence. In their work, \cite{Gu0XLS18} employs Noisy parallel decoding (NPD), which generates multiple predictions of different lengths with fertility, and then a pretrained AT model is used to rescore them. Because NPD is still quite requires additional parameters, \cite{stern19a,GuWZ19}  applied insertion method, which is partially autoregressive and uses the insertion operations for more flexible and dynamic length changes. \cite{shu2020latent} refines the latent variables instead of the tokens, allowing for dynamically adaptive prediction length. \cite{libovicky-helcl-2018-end} introduces CTC \cite{GravesFGS06}, which is a latent alignment model to utilize a sequence of discrete latent alignment variables to align the NMT monotonically. This work uses CTC to solve the target length problem and proposes CTC upsampling strategy to improve performance.  
\subsection{Knowledge Distillation}
Another main problem is the multi-modal. NAT removes the conditional dependence between target tokens and predicting the independent issue leads to multi-modal outputs and induces the repetition of tokens. A standard approach to overcome the multi-modality problem is to use sequence-level knowledge distillation \cite{kim-rush-2016-sequence}, by replacing the target side of the training set with the output from an AT model. Various advanced model architectures \cite{lee-etal-2018-deterministic,ghazvininejad-etal-2019-mask} use iteration-based methods that can see the previous or partially predicted tokens to add dependence to solve the multi-modal problem. This work explores an alternative paradigm: we use not only strong AT teacher in sequence-level knowledge distillation but also leverage contextualized PMLM in target to learn the information from pretraining.

\subsection{PMLM Initialization}
There have been some pretrained encoder-decoder-based multilingual language models \cite{lample2019cross,zanon-boito-etal-2020-mass,liu-etal-2020-multilingual-denoising,xue-etal-2021-mt5,li-etal-2022-universal} that achieve superior translation performance. Most of them are dedicated to AT, while \cite{li-etal-2022-universal} intends to pretrain models that can be applied to both AT and NAT. Some \cite{rothe-etal-2020-leveraging, lample2019cross, Zhu2020Incorporating, 10.5555/3495724.3496634} otherwise incorporate encoder-based pretrained multilingual language models (PMLMs) into encoder-decoder-based transformer AT models for better translation performance. \cite{li-etal-2022-universal, Zhu2020Incorporating, 10.5555/3495724.3496634,su-etal-2021-non} utilizes PMLMs to initialize NAT models. Among them, \cite{li-etal-2022-universal, Zhu2020Incorporating, 10.5555/3495724.3496634} are iterative models with strong performance while \cite{su-etal-2021-non} is one-pass with weaker performance. This work instead directly finetunes PMLMs with CTC as one-pass models for faster inference, yet with comparable or better performance with respect to PMLM-initialized iterative NAT models. %We freeze the word embedding and output projection layer to keep pretraining knowledge to improve performance further.


% Their results on the major NAT benchmarks WMT'14 En$\leftrightarrow$De vary because of different AT teachers (transformer base or transformer big). Thus it isn't easy to deduce which is better since the most common baseline architecture is transformer base, and it would not be a fair comparison. Meanwhile, \cite{shao2022nmla} surpasses the baseline models on both WMT'14 En$\leftrightarrow$De and WMT'16 en$\leftrightarrow$ro without initializing from PMLMs. It sets the new record for non-iterative NAT models trained on distillation data from transformer base teachers.
